Metrology of open quantum systems from emitted radiation

We explore the task of learning about the dynamics of a Markovian open quantum system by monitoring the information it radiates into its environment. For an open system with Hilbert space dimension $D$, the quantum state of the emitted radiation can be described as a temporally ordered matrix-product state (MPS). We provide simple analytical expressions for the quantum Fisher information (QFI) of the radiation state, which asymptotically scales linearly with the sensing time unless the open system has multiple steady states. We characterize the crossovers in QFI near dynamical phase transitions, emphasizing the role of temporal correlations in setting the asymptotic rate at which QFI increases. We discuss when optimal sensing is possible with instantaneously measured radiation.

==> Full_QFI.tex <==
\section{Joint QFI}
Now, we pay attention to the full output state upon $t$ iterations of the isometry $V$. Starting from the system state $\ket{\psi} \in \mathcal{H}_D$, we have the state at time $t$ denoted $\ket{\Psi;t} \in \C^{D\times d^t}$ as,
\begin{align}
    \ket{\Psi;t} = \quad
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
        \GTensor{0,0}{1.2}{.6}{\small $V$}{7};
      \GTensor{1*\singledx,0}{1.2}{.6}{\small $V$}{7};
      \GTensor{2*\singledx,0}{1.2}{.6}{\small $V$}{7};
      \GTensor{3*\singledx,0}{1.2}{.6}{\small $V$}{7};
      \GTensor{4*\singledx,0}{1.2}{.6}{\small $V$}{7};
    \DTensor{5*\singledx,0}{1.2}{.6}{\small ${\psi}$}{7};
\end{tikzpicture}
    \quad 
\end{align}
We recall that the initial state is not parameter-dependent. Thus, we have
\begin{align}
\partial_\theta\ket{\Psi;t} = \mathlarger{\sum}_{\tau=1}^t    \quad\dots
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
        \GTensor{0,0}{1.2}{.6}{\small $V_L$}{7};
      \GTensor{1*\singledx,0}{1.2}{.6}{\small $V_L$}{7};
      \draw (1*\singledx,-1.8) node {\small $m_{\tau-1}$};
      \GTensor{2*\singledx,0}{1.2}{.6}{\scriptsize $\partial_\theta V_{C}$}{7};
      \draw (2*\singledx,-1.8) node {\small $m_{\tau}$};
      \GTensor{3*\singledx,0}{1.2}{.6}{\small $V_R$}{7};
      \draw (3*\singledx,-1.8) node {\small $m_{\tau+1}$};
      \GTensor{4*\singledx,0}{1.2}{.6}{\small $V_R$}{7}
      \DTensor{5*\singledx,0}{1.2}{.6}{\small ${\psi}$}{7};
\end{tikzpicture}
    \quad 
\end{align} 
The QFI is given as,
\begin{equation}
    F_{SE}(t;\psi,\theta,V) = 4\left(\inner{\partial_\theta\Psi;t}{\partial_\theta\Psi;t} - |\inner{\partial_\theta\Psi;t}{\Psi;t}|^2\right)
\end{equation}
Now,
\begin{align}
\underset{\psi \sim \mu_H}{\mathbb{E}}\quad
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
\GFTensor{0,2}{1.2}{.6}{\small $\partial_\theta V$}{1};
\GFTensor{0,0}{1.2}{.6}{\small $\partial_\theta \bar{V}$}{0};
\draw (1,1) node {\small \dots};
\draw[very thick,draw=red] (-1.2,0)--(-1.2,2);
\DTensor{3.6,0}{1.2}{.6}{\small $\bar{\psi}$}{7};
\DTensor{3.6,2}{1.2}{.6}{\small ${\psi}$}{7};
\end{tikzpicture}
  =   \frac{1}{D}\quad
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
\GFTensor{0,2}{1.2}{.6}{\small $\partial_\theta V$}{1};
\GFTensor{0,0}{1.2}{.6}{\small $\partial_\theta \bar{V}$}{0};
\draw (1,1) node {\small \dots};
\draw[very thick,draw=red] (-1.2,0)--(-1.2,2);
\draw[very thick,draw=red] (3,0)--(3,2);
\end{tikzpicture}
\end{align} 

\begin{align}
&\underset{\psi \sim \mu_H}{\mathbb{E}}\quad
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
\GFTensor{0,2}{1.2}{.6}{\small $\partial_\theta V$}{1};
\GFTensor{0,0}{1.2}{.6}{\small $\bar{V}$}{0};
\draw (1,1) node {\small \dots};
\draw[very thick,draw=red] (-1.2,0)--(-1.2,2);
\DTensor{3.6,0}{1.2}{.6}{\small $\bar{\psi}$}{7};
\DTensor{3.6,2}{1.2}{.6}{\small ${\psi}$}{7};
\GFTensor{0,-2}{1.2}{.6}{\small $V$}{1};
\GFTensor{0,-4}{1.2}{.6}{\small $\partial_\theta\bar{V}$}{0};
\draw (1,-3) node {\small \dots};
\draw[very thick,draw=red] (-1.2,-4)--(-1.2,-2);
\DTensor{3.6,-4}{1.2}{.6}{\small $\bar{\psi}$}{7};
\DTensor{3.6,-2}{1.2}{.6}{\small ${\psi}$}{7};
\end{tikzpicture} \quad =  \\ & \\ 
&\frac{1}{D(D+1)}\left(\quad
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
\GFTensor{0,2}{1.2}{.6}{\small $\partial_\theta V$}{1};
\GFTensor{0,0}{1.2}{.6}{\small $\bar{V}$}{0};
\draw (1,1) node {\small \dots};
\draw[very thick,draw=red] (-1.2,0)--(-1.2,2);
\draw[very thick,draw=red] (3,0)--(3,2);
\GFTensor{0,-2}{1.2}{.6}{\small $V$}{1};
\GFTensor{0,-4}{1.2}{.6}{\small $\partial_\theta\bar{V}$}{0};
\draw (1,-3) node {\small \dots};
\draw[very thick,draw=red] (-1.2,-4)--(-1.2,-2);
\draw[very thick,draw=red] (3,-4)--(3,-2);
\end{tikzpicture}
  \quad  +  \quad 
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
\GFTensor{0,2}{1.2}{.6}{\small $\partial_\theta V$}{1};
\GFTensor{0,0}{1.2}{.6}{\small $\bar{V}$}{0};
\draw (1,1) node {\small \dots};
\draw[very thick,draw=red] (-1.2,0)--(-1.2,2);
\GFTensor{0,-2}{1.2}{.6}{\small $V$}{1};
\GFTensor{0,-4}{1.2}{.6}{\small $\partial_\theta\bar{V}$}{0};
\draw (1,-3) node {\small \dots};
\draw[very thick,draw=red] (-1.2,-4)--(-1.2,-2);
\draw[very thick,draw=red] (3,0)--(3,-2);
\draw[very thick,draw=red] (4,2)--(4,-4);
\draw[very thick,draw=red] (3,2)--(4,2);
\draw[very thick,draw=red] (3,-4)--(4,-4);
\end{tikzpicture} \quad\right)
\end{align} 

We thus define,

\begin{align}\label{eq:alphatwiddle}
  \tilde{\alpha}(t) := \quad
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
      \GTensor{0,0}{1.2}{.6}{\scriptsize $\partial_\theta V$}{7};
      \GTensor{0,-2}{1.2}{.6}{\scriptsize $\partial_\theta \bar{V}$}{0};
      % \draw[very thick,draw=red] (1.2,0)--(2.03,0);
    \FUnitary{1.75,-2.25}{1}{.6}{\small $\sum T$}{6};
        \draw[very thick,draw=red] (2.355,0)--(3.5,0);
        \draw[very thick,draw=red] (2.355,-2)--(3.5,-2);
        \draw[very thick,draw=red] (3.5,-2)--(3.5,0);
        \draw[very thick,draw=red] (-2,0)--(-1.2,0);
        \draw[very thick,draw=red] (-2,-2)--(-1.2,-2);
        \draw[very thick,draw=red] (-2,-2)--(-2,0);
\end{tikzpicture}
    \quad 
\end{align} 

\begin{align}\label{eq:gammatwiddle}
  \tilde{\gamma}(t) := \quad
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
      \GTensor{0,0}{1.2}{.6}{\scriptsize $\partial_\theta V$}{7};
      \GTensor{0,-2}{1.2}{.6}{\scriptsize $\bar{V}$}{0};
      % \draw[very thick,draw=red] (1.2,0)--(2.03,0);
    \FUnitary{1.75,-2.25}{1}{.6}{\small $\sum T$}{6};
        \draw[very thick,draw=red] (2.355,0)--(3.5,0);
        \draw[very thick,draw=red] (2.355,-2)--(3.5,-2);
        \draw[very thick,draw=red] (3.5,-2)--(3.5,0);
        \draw[very thick,draw=red] (-2,0)--(-1.2,0);
        \draw[very thick,draw=red] (-2,-2)--(-1.2,-2);
        \draw[very thick,draw=red] (-2,-2)--(-2,0);
\end{tikzpicture}
    \quad 
\end{align} 
where $\sum T:= \sum_{\tau = 0}^{t-1} T_V^\tau$.
\begin{align}\label{eq:betastwiddle}
 \tilde{\beta}_\tau(t) := \quad
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
      \GTensor{-5,0}{1.2}{.6}{\scriptsize $\partial_\theta V$}{7};
      \GTensor{-5,-2}{1.2}{.6}{\small $\bar{V}$}{0};
        \draw[very thick,draw=red] (-5-1.15,-2)--(-5-1.15,0);
        \FUnitary{-3.25,-2.25}{1}{.6}{\small $T_V^\tau$}{5};
      \GTensor{-1.45,0}{1.2}{.6}{\small ${V}$}{7};
      \GTensor{-1.45,-2}{1.2}{.6}{\scriptsize $\partial_\theta \bar{V}$}{0};
          \draw[very thick,draw=red] (-0.5,-2)--(0.15,-2);
          \draw[very thick,draw=red] (-0.5,0)--(0.15,0);
    \FUnitary{0.75,-2.25}{1}{.6}{\small $M_{\tau}$}{6};
        \draw[very thick,draw=red] (1.35,0)--(2,0);
        \draw[very thick,draw=red] (1.35,-2)--(2,-2);
        \draw[very thick,draw=red] (2,-2)--(2,0);
      \end{tikzpicture}
    \quad
\end{align} 
where $M_{\tau} := 2\sum_{\tau'=0}^{t-2-\tau}T_V^{\tau'}$.

\begin{align} \label{eq:deltatwiddle}
 \tilde{\delta}_\tau(t) := \quad
\begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
      \GTensor{-5,0}{1.2}{.6}{\scriptsize $\partial_\theta V$}{7};
      \GTensor{-5,-2}{1.2}{.6}{\small $\bar{V}$}{0};
        \draw[very thick,draw=red] (-5-1.15,-2)--(-5-1.15,0);
        \FUnitary{-3.25,-2.25}{1}{.6}{\small $T_V^\tau$}{5};
      \GTensor{-1.45,0}{1.2}{.6}{\small $\partial_\theta\bar{V}$}{7};
      \GTensor{-1.45,-2}{1.2}{.6}{\scriptsize $V$}{0};
          \draw[very thick,draw=red] (-0.5,-2)--(0.15,-2);
          \draw[very thick,draw=red] (-0.5,0)--(0.15,0);
    \FUnitary{0.75,-2.25}{1}{.6}{\small $N_{\tau}$}{6};
        \draw[very thick,draw=red] (1.35,0)--(2,0);
        \draw[very thick,draw=red] (1.35,-2)--(2,-2);
        \draw[very thick,draw=red] (2,-2)--(2,0);
      \end{tikzpicture}
    \quad, 
\end{align} 
where $N_{\tau} = \sum_{\tau' = 0}^{\min\{\tau,2(t-1)-\tau\}}T_V^{\tau'}$



With this, we state the next result.
\begin{coloredtheorem}[Expected Joint QFI] \label{re:totqfinormalmps}
With the same setting as Result \ref{re:qfinormalmps}, we have the QFI of the joint system and emission field state, $\langle F_{SE}\rangle \equiv \underset{\psi \sim \mu_H}{\mathbb{E}} F_{SE}(t;\psi,\theta,V)$
\begin{align}
   \langle F_{SE}\rangle &= 
    4 \left( \frac{1}{D} \left[ \tilde{\alpha}(t) + \sum_{\tau=0}^{t-2} \tilde{\beta}_\tau(t) \right] \right. \\
    &\quad \left. - \frac{1}{D(D+1)} \left[ |\tilde{\gamma}(t)|^2 + \sum_{\tau=0}^{2(t-1)} \tilde{\delta}_\tau(t) \right] \right) \end{align}
where the expectation is taken over the Haar measure on the input state space $\mathcal{H}_D$, and $\tilde{\alpha}(t), \tilde{\beta}(t),\tilde{\gamma}(t),\tilde{\delta}(t)$ are defined as in \cref{eq:alphatwiddle,eq:betastwiddle,eq:gammatwiddle,eq:deltatwiddle}.
\end{coloredtheorem}

\begin{corollary}\label{cor:totQFIbound}
    For an Liouivillian generating irreducible dynamics, the asymptotic scaling of the joint QFI $F_{SE}$ is identical to that of the emission QFI $F_E$.
\end{corollary}

We note that $\tilde{\alpha}(t) \to D\alpha t$, $\tilde{\gamma}(t) \to D\gamma t$, $\sum_{\tau \leq t-2}\tilde{\beta}_\tau(t) \to (t^2 - t)|\gamma|^2D$, and $\sum_{\tau \leq 2(t-1)}\tilde{\delta}_\tau(t) \to t^2 D|\gamma|^2$. Thus, the asymptotic scaling is,
\begin{align}
    &4\left(\frac{D\alpha t + (t^2 - t)|\gamma|^2 D}{D} - \frac{D^2 |\gamma|^2 t^2 + t^2 D |\gamma|^2}{D(D + 1)}\right) \\
    &\to 4\left( \alpha - |\gamma|^2 \right)t
\end{align}

We summarise this as follows,

\begin{equation} 
\begin{array}{rcl}
&\text{Total QFI = } \tilde{O}(t)   \Leftrightarrow \text{MPS QFI = } \tilde{O}(t)  \\ & \hspace{-25mm}\Searrow  &
\\& \text{Noisy QFI = } \tilde{O}(t)
\end{array}
\end{equation}
% \begin{align} \label{eq:deltanormal}
%   \delta_\infty \equiv \quad
% \begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
%       \GTensor{-5,0}{1.2}{.6}{\scriptsize $\partial_\theta V$}{7};
%       \GTensor{-5,-2}{1.2}{.6}{\small $\bar{V}$}{0};
%         \draw[very thick,draw=red] (-5-1.15,-2)--(-5-1.15,0);
%             \DTensor{-3.5,-1}{1.}{.6}{\small $\rho_{ss}$}{1};
%         \draw[very thick,draw=red] (-4,-2)--(-3.5,-2);
%             \draw[very thick,draw=red] (-4,0)--(-3.5,0);
%       \GTensor{-1.,0}{1.2}{.6}{\scriptsize $\partial_\theta\bar{V}$}{7};
%       \GTensor{-1.,-2}{1.2}{.6}{\scriptsize ${V}$}{0};
%           \draw[very thick,draw=red] (0.25,0)--(0.25,-2);
%         \draw[very thick,draw=red] (-2.2,0)--(-2.2,-2);
%       \end{tikzpicture}
%     \quad = \quad \gamma \times
% \begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
%       \GTensor{-1.,0}{1.2}{.6}{\scriptsize $\partial_\theta\bar{V}$}{7};
%       \GTensor{-1.,-2}{1.2}{.6}{\scriptsize ${V}$}{0};
%           \draw[very thick,draw=red] (0.25,0)--(0.25,-2);
%         \draw[very thick,draw=red] (-2.2,0)--(-2.2,-2);
%       \end{tikzpicture} \quad 
% \end{align} 


An implication of this bound is that for an ergodic system, entanglement in the initial state cannot act as a resource for Heisenberg limited sensing, either of the full state or in the case of noisy metrology.
% % \begin{equation}
% % \mathbb{E}_{\psi\sim\mu_H}\inner{\partial_\theta\psi;t}{\partial_\theta\psi;t} = \frac{\inner{\partial_\theta V}{\partial_\theta V}}{D}
% % \end{equation}
% % \begin{equation}
% % \mathbb{E}_{\psi\sim\mu_H}|\inner{\partial_\theta\psi;t}{\psi;t}|^2 = 
% % \end{equation}
% \textcolor{red}{\textit{Conjecture}. $\gamma$ goes as $1/D$.}

==> noninjective.tex <==
\section{Non-injective joint QFI}
Let us now examine the long-time value, restricting ourselves to the case of stationary dynamics by fixing $\Delta=0$, and denoting the steady-state subspace degenerecy with $\mu,\nu\in [d_{\text{ss}}]$. With this restriction, we note that $\Psi_\nu$ and $J^\mu$ can be made Hermitian, along with the biorthogonality $\llangle J^\mu|\Psi_\nu\rrangle = \delta^\mu_\nu$. We denote $\Gamma^{\mu}_{\nu} \equiv \Gamma^{\mu,0}_{\nu,0}$.
%  Now, using the fact that the eigenoperators are Hermitian (also implying that $c_\mu \in \mathbb{R}$), we note that   
\begin{eqnarray}
    |\gamma|^2 = \sum_{\mu\nu}c_\mu {c}_\nu\Gamma_\mu^\mu\bar{\Gamma}_\nu^\nu %= |\text{Tr}(\Gamma)|^2
\end{eqnarray}
and 
\begin{eqnarray}
    \beta_{\infty} = \sum_{\mu\nu} c_\mu\Gamma^{\mu}_\nu \bar{\Gamma}^\nu_\mu %= \text{Tr}(\bar{\Gamma}\Gamma)
\end{eqnarray}
The optimal scaling is achieved by the following optimization over the initial state-dependent coefficients,
\begin{eqnarray}
    \underset{\mathbf{c}\in \C^{d_{\text{ss}}}}{\max} \sum_{\mu,\nu \in d_{\text{ss}}}\left(c_\mu\Gamma^{\mu}_\nu \bar{\Gamma}^\nu_\mu - c_\mu {c}_\nu\Gamma_\mu^\mu\bar{\Gamma}_\nu^\nu\right)
\end{eqnarray}
The `diagonal' part of this expression is,
\begin{eqnarray}
    \sum_{\mu \in d_{\text{ss}}} c_\mu(1-c_\mu) |\Gamma_\mu^\mu|^2
\end{eqnarray}
Whereas, the `off-diagonal' contribution is,
\begin{eqnarray}
    \sum_{\mu\neq\nu \in d_{\text{ss}}} c_\mu \left(\Gamma^{\mu}_\nu \bar{\Gamma}^\nu_\mu -  {c}_\nu\Gamma_\mu^\mu\bar{\Gamma}_\nu^\nu\right)
\end{eqnarray}

% \begin{eqnarray}
%     \Gamma^{\mu}_\nu \bar{\Gamma}^\nu_\mu -  {c}_\nu\Gamma_\mu^\mu\bar{\Gamma}_\nu^\nu \geq \Gamma^{\mu}_\nu \bar{\Gamma}^\nu_\mu -  \Gamma_\mu^\mu\bar{\Gamma}_\nu^\nu
% \end{eqnarray}


Recalling the injective case, we note that the off-diagonal part is null and the diagonal part has only $c_{\mu^*} = 1$ and vanishes. Thus, we re-gain the previous result with this calculation. Back to the long-range MPS, we choose a basis of the steady-state manifold such that $0 \leq J^\mu \leq \mathbbm{1}$ which ensures $c_\mu \in [0,1]$ (see Appendix~\ref{sec:statbasisprops}). This implies that a sufficient condition for the diagonal part to be positive and bounded away from zero is to have a non-trivial distribution of $\mathbf{c} = (c_\mu)_\mu$.


\begin{align} 
    \tilde{\alpha} := \sum_\mu \text{Tr}[J^\mu] \quad
  \begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
        \GTensor{0,0}{1.2}{.6}{\scriptsize $\partial_\theta V$}{7};
        \GTensor{0,-2}{1.2}{.6}{\scriptsize $\partial_\theta \bar{V}$}{0};
        \draw[very thick,draw=red] (1.2,0)--(2.03,0);
      \DTensor{2,-1}{1.}{.6}{\small $\Psi_\mu$}{1};
            \draw[very thick,draw=red] (1.2,-2)--(2.03,-2);
          \draw[very thick,draw=red] (-2,0)--(-1.2,0);
          \draw[very thick,draw=red] (-2,-2)--(-1.2,-2);
          \draw[very thick,draw=red] (-2,-2)--(-2,0);
  \end{tikzpicture}
      \quad 
  \end{align} 

  \begin{align} 
    \tilde{\gamma} := \sum_\mu \text{Tr}[J^\mu] \quad
  \begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
        \GTensor{0,0}{1.2}{.6}{\scriptsize $\partial_\theta V$}{7};
        \GTensor{0,-2}{1.2}{.6}{\small $\bar{V}$}{0};
        \draw[very thick,draw=red] (1.2,0)--(2.03,0);
      \DTensor{2,-1}{1.}{.6}{\small $\Psi_\mu$}{1};
            \draw[very thick,draw=red] (1.2,-2)--(2.03,-2);
          \draw[very thick,draw=red] (-2,0)--(-1.2,0);
          \draw[very thick,draw=red] (-2,-2)--(-1.2,-2);
          \draw[very thick,draw=red] (-2,-2)--(-2,0);
  \end{tikzpicture}
      \quad 
  \end{align} 



  \begin{align} 
    \tilde{\beta} := \sum_{\mu,\nu,\Delta} \text{Tr}[J^\mu]e^{\iota t \Delta} \quad
    \begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
          \GTensor{0,0}{1.2}{.6}{\scriptsize $\partial_\theta V$}{7};
          \GTensor{0,-2}{1.2}{.6}{\small $\bar{V}$}{0};
          \draw[very thick,draw=red] (1.2,0)--(2.03,0);
        \DTensor{2,-1}{1.}{.6}{\small $\Psi_{\nu\Delta}$}{1};
              \draw[very thick,draw=red] (1.2,-2)--(2.03,-2);
            \draw[very thick,draw=red] (-2,0)--(-1.2,0);
            \draw[very thick,draw=red] (-2,-2)--(-1.2,-2);
            \draw[very thick,draw=red] (-2,-2)--(-2,0);
            \begin{scope}[xshift=6cm]
              \GTensor{0,0}{1.2}{.6}{\small $V$}{7};
              \GTensor{0,-2}{1.2}{.6}{\scriptsize $\partial_\theta\bar{V}$}{0};
              \draw[very thick,draw=red] (1.2,0)--(2.03,0);
            \DTensor{2,-1}{1.}{.6}{\small $\Psi_{\mu}$}{1};
                  \draw[very thick,draw=red] (1.2,-2)--(2.03,-2);
                \draw[very thick,draw=red] (-2,0)--(-1.2,0);
                \draw[very thick,draw=red] (-2,-2)--(-1.2,-2);
            \UTensor{-2,-1}{1.}{.6}{\small $J^{\nu\Delta}$}{1};          
            \end{scope}
    \end{tikzpicture}
        \quad 
  \end{align} 

  \begin{align} 
    \tilde{\delta} := \sum_{\mu,\nu,\Delta} \text{Tr}[J^\mu]e^{\iota t \Delta} \quad
  \begin{tikzpicture}[scale=0.5,baseline={([yshift=-0.65ex] current bounding box.center) }]
        \GTensor{0,0}{1.2}{.6}{\scriptsize $\partial_\theta V$}{7};
        \GTensor{0,-2}{1.2}{.6}{\small $\bar{V}$}{0};
        \draw[very thick,draw=red] (1.2,0)--(2.03,0);
      \DTensor{2,-1}{1.}{.6}{\small $\Psi_{\nu\Delta}$}{1};
            \draw[very thick,draw=red] (1.2,-2)--(2.03,-2);
          \draw[very thick,draw=red] (-2,0)--(-1.2,0);
          \draw[very thick,draw=red] (-2,-2)--(-1.2,-2);
          \draw[very thick,draw=red] (-2,-2)--(-2,0);
          \begin{scope}[xshift=6cm]
            \GTensor{0,0}{1.2}{.6}{\scriptsize $\partial_\theta \bar{V}$}{7};
            \GTensor{0,-2}{1.2}{.6}{\small $V$}{0};
            \draw[very thick,draw=red] (1.2,0)--(2.03,0);
          \DTensor{2,-1}{1.}{.6}{\small $\Psi_{\mu}$}{1};
                \draw[very thick,draw=red] (1.2,-2)--(2.03,-2);
              \draw[very thick,draw=red] (-2,0)--(-1.2,0);
              \draw[very thick,draw=red] (-2,-2)--(-1.2,-2);
          \UTensor{-2,-1}{1.}{.6}{\small $J^{\nu\Delta}$}{1};          
          \end{scope}
  \end{tikzpicture}
      \quad 
  \end{align} 




  
